TorchQL: A Programming Framework for Integrity Constraints in Machine Learning

Finding errors in machine learning applications requires a thorough exploration of their behavior over data. Existing approaches used by practitioners are often ad-hoc and lack the abstractions needed to scale this process. We present TorchQL, a programming framework to evaluate and improve the correctness of machine learning applications. TorchQL allows users to write queries to specify and check integrity constraints over machine learning models and datasets. It seamlessly integrates relational algebra with functional programming to allow for highly expressive queries using only eight intuitive operators. We evaluate TorchQL on diverse use-cases including finding critical temporal inconsistencies in objects detected across video frames in autonomous driving, finding data imputation errors in time-series medical records, finding data labeling errors in real-world images, and evaluating biases and constraining outputs of language models. Our experiments show that TorchQL enables up to 13x faster query executions than baselines like Pandas and MongoDB, and up to 40% shorter queries than native Python. We also conduct a user study and find that TorchQL is natural enough for developers familiar with Python to specify complex integrity constraints.

==> limitations.tex <==
\section{Limitations and Future Work}

Talk about limitations of \tool{}: it is built as an in-memory dataset, it is implemented in Python, it is not
optimized for distributed execution, etc.
Tie them into opportunities for future work.
Talk about how we can extend \tool{} to support features like query recursion, and how we can extend \tool{} to
support differentiable queries that can be used to monitor the training progress of models.

Some of the limitations of the system include:
\begin{enumerate}[leftmargin=*]
    \item Parallelism: \tool{} does not perform processes concurrently or parallelly and does not take advantage of multicore systems with the exception of loading data into the database. However, we leave this as future work. The structure of the system makes it highly amenable to parallelism by integrating multiprocessing components into the abstractions provided by \tool{}.
    \item In-Memory Database: \tool's database is in-memory. This means that any data being queried over is limited by the size of the RAM of the system, limiting the ability of \tool{} to query over larger amounts of data. Traditionally databases are not in-memory to prevent this problem with scalability, and load chunks of data as needed, but this results in a loss of performance during the I/O operations associated with reading from and writing to disk.
    \item Support for Synthesis: \tool{} is currently a new library and it is therefore harder to synthesize \tool{} queries than typical Python. However, we have obtained some initial success via few shot prompting where GitHub's Copilot and GPT-4 are able to synthesize some queries after giving examples. To help with the interactive nature of debugging, additional support for synthesis, such as the ability to synthesize UDFs or just the query structure is an area of future work.
\end{enumerate}


==> motifs.tex <==
\section{Motifs}

\begin{enumerate}
    \item Talk about the general motifs for \framework{}
    \begin{enumerate}
        \item Registering a PyTorch Dataset
        \item Dumping model predictions, along with GPU support
        \item Extracting features from unstructured data
        \item Structuring schema out of those features
    \end{enumerate}
\end{enumerate}

